Cobordism, Singularities and the Ricci Flow Conjecture

In the following work, an attempt to conciliate the Ricci flow conjecture and the Cobordism conjecture, stated as refinements of the Swampland distance conjecture and of the No global symmetries conjecture respectively, is presented. This is done by starting from a suitable manifold with trivial cobordism class, applying surgery techniques to Ricci flow singularities and trivialising the cobordism class of one of the resulting connected components via the introduction of appropriate defects. The specific example of $\Omega^{SO}_4$ is studied in detail. A connection between the process of blowing up a point of a manifold and that of taking the connected sum of such with $\mathbb{CP}^n$ is explored. Hence, the problem of studying the Ricci flow of a $K3$ whose cobordism class is trivialised by the addition of $16$ copies of $\mathbb{CP}^2$ is tackled by applying both the techniques developed in the previous sections and the classification of singularities in terms of ADE groups.

==> bin.tex <==
\subsection{On blowups and magnetic monopoles (OLD)}

Note: I am keeping this as a template: now that I am more comfortable with the paper I want to structure this differently

One publication which might shed some light on the connected sum of 16 $\mathbb{CP}^2$ which we were forced to consider for the trivialization of the cobordism class of $K3$ could be \cite{nCP2s}. In it, an explicit example of a self-dual metric on the connected sum of $n$ copies of $\mathbb{CP}^2$ is given. Furthermore, it is precisely obtained as the blow-up of $n$ singularities, which are then interpreted (due to the \textit{ansatz} used by the author), as magentic monopoles on hyperbolic space. This is interesting, since we could make a connection between the connected sum of copies of $\mathbb{CP}^2$ and the presence of branes transverse to $K3$. This setup is familiar from the elliptic fibration which is the starting point of F-theory, and the singularities which any such elliptic fibration is forced to have is precisely given by transverse $D7$-branes.

Going back to \cite{nCP2s}, we would like to apply the Ricci flow machinery to some metric, in order to see if this gives us any information on the behavior or appeareance of the singularities. However, the problem is that the metric is not given in an explicit global way, but rather in terms of some connection form $\omega$. This is because the author first considers a general scalar-flat Kähler metric on a circle bundle over some open set in $\mathbb{R}^3$. The key feature of this class of metrics is that they are defined by solutions of Laplace equations. Then, the paper goes on to consider a very explicit metric, called the Burns metric, which describes a blowup at the origin of $\mathbb{C}^2$. I will come back to this later. The key argument is that this metric can be recast as one of the aforementioned metrics. In particular, the Laplace equation which defines the metric is given in terms of the metric of hyperbolic 3-space $\mathcal{H}$, namely
\begin{equation}
    h=\frac{dx^2+dy^2+dq^2}{q^2}, \hspace{1cm}\text{where} \ q>0
\end{equation}
Given coordinates $(x,y,z)$ on $H^3=\{(x,y,z)\in \mathbb{R}^3 \mid z>0\}$, and setting $q=\sqrt{2z}$, the whole metric (or a representative of its conformal class) is given by
\begin{equation}\label{eq:gburns}
    g=Vh+V^{-1}\omega
\end{equation}
where $V=2zf$, $f$ satisfies
\begin{equation}
    f_{xx}+f_{yy}+(2zf)_{zz}=0,
\end{equation}
adn finally, $\omega$ is a connection form on a circle bundle, on which there is only a restriction on the associated curvature, which is required to be $*dV$.

The problem with \eqref{eq:gburns} is that it is not very computationally firendly when applying globally defined equations. This is because in order to give coordinates associated to the fourth dimension, we require a trivialization of the circle bundle, which is local procedure. Nonetheless, said metric allows the author to give an explicit expression for $V$ in terms of the fundamental solution (Green's function) of the Laplace-Beltrami operator relative to the hyperbolic volume form $G$, namely
\begin{equation}\label{eq:V}
    V=1+G; \hspace{1cm}, \text{where} \ G=\frac{1}{e^{2\rho}-1},
\end{equation}
where $\rho$ is some (hyperbolic) distance from $(0,0,q_0)$ (interpreted as the location of the magnetic monopole), and some other generic point in hyperbolic 3-space. This observation is what led the author to consider a generic $V$ made up of a superposition of Green's functions for multiple locations of magnetic monopoles.

In particular, to construct a metric for the connected sum of $n$ copies of $C\mathbb{P}^2$, one needs to consider a total of $n$ such magnetic monopoles. At the level of the metric, this translates into $n$ singular loci of the base $\mathcal{H}^3$ over which the circle bundle degenerate. Thus, one needs to consider a set of $n$ singular points $p_j\in \mathcal{H}^3$, and for each of them a Green's function $G_j$, so that the total $V$ which enters the metric is given by 
\begin{equation}\label{eq:Vtotal}
    V=1+\sum_{i=1}^n\frac{1}{e^{2\rho_i}-1}
\end{equation}

A further problem of this construction is that the given metric is not directly the metric on $\mathbb{CP}^2\#\ldots\#\mathbb{CP}^2$, but rather a metric which is in the same conformal class as a self-dual metric on said space. The good news is that this might not be such a hurdle, as the article itself proposes a candidate for a metric which is not scalar-flat, and can therefore be a candidate for an explicit metric on $\mathbb{CP}^2\#\ldots\#\mathbb{CP}^2$ itself. Said rescaling is again given in terms of the conformal distance from an arbitrary point in hyperbolic 3-space:
\begin{equation}\label{eq:ncp2metric}
    g=(\text{sech}^2(\rho))\left[Vh+V^{-1}\omega^2\right]
\end{equation}
Again, we are met with the presence of the connection one-form $\omega$ corresponding to a circle bundle, which complicates the application of the Ricci flow.








\section{Davide's outlook}
In our work, the powerful tools offered by surgery techniques for singular geometric flow equations, as those introduced by Perelman, and blow-up procedures in algebraic geometry were jointly applied in the context of the Cobordism conjecture. After having introduced the appropriate mathematical apparatus, it was argued -and explicitly shown for the simple cases of Einstein manifolds and Ricci solitons- that Ricci flow preserves Ponryagin and Stiefel-Whitney numbers. Since such invariants unambiguously fix an element of $\Omega_4^{SO}$, the above statement implies that Ricci flow preserves the corresponding cobordism class. Thereafter, our attention was moved to surgery procedures, which are applied by taking a portion of a connected component of a flowing manifold where a pinching would occur along Ricci flow and substituting it with two smooth caps, so that two connected components with a well-defined flow behaviour are produced. It can be shown that the resulting manifold is cobordant to the original one, so that surgeries preserve cobordism classes. It is nevertheless interesting and reasonable, from a more physical perspective, to investigate the effects of completely removing one of the two components resulting from the surgery. In general, this can imply the necessity of balancing such a modification out by the introduction of defects, that mimic the contribute of the removed component to the overall cobordism class. Therefore, focusing on the specific string-theory inspired example of a $K3$, it was argued that its cobordism class can be trivialised by adding to it, either via a disjoint union or a connected sum, the connected sum of 16 copies of $\mathbb{CP}^2$. Alternatively, the result can be obtained by making the manifold singular. In the last sections, the two equivalent possibilities were presented and studied. Indeed, it was shown that one can go from the further to latter by connecting the $\mathbb{CP}^2$s to the $K3$ with appropriate throats and allowing them to pinch along Ricci flow, while the opposite can be achieved by blowing-up the singularities. The Ricci flow of a connected sum of $\mathbb{CP}^2$s, endowed with the so-called Burns metric, was examined in detail. In the end, ADE groups were introduced as a useful tool to characterise the feature of the previously mentioned singularities. This was done by the means of lattice polarizations. The most natural prosecution of our analysis would be to consider more complicated cobordism structures, such as $\Omega_d^{\text{Spin}}$ or $\Omega_d^{\text{String}}$, but this goes way beyond the scope of the current work.




------------------------------------------------------------------------------

\subsection{The Ricci flow equations for the Burns metric}
An alternative route to try to learn more about the behavior of the $n\mathbb{CP}^2$ manifold under the Ricci flow is to look not to the full, complicated metric in \eqref{eq:lametrica2}, but to the Burns metric. This is motivated by the complicated nature of the full metric, but also by what the Burns metric describes. As we have stated on multiple instances, the Burns metric describes a Scalar-flat K\"ahler geometry on the blowup of $\mathbb{C}^2$ at the origin. While the scalar-flatness negates the argument from the above sections, the explicit nature of the metric allows us to produce explicit calculations, and see how the geometry evolves under the flow. In particular, we will be interested in the geometry around the origin, where the so-called \textit{exceptional divisor}\footnote{I will probably explain this either before or after this section.} is located. Again, because of the diffeomorphism of a blow-up of a manifold at a point and its connected sum with a complex projective space (in the dimensionality at hand, this is a $\mathbb{CP}^2$), the case of the Burns metric seems relevant to our scenario.

We begin by writing down the explicit form of the Burns metric. To this, end we start from \eqref{eq:burnscoord}, and use the explicit expression of the $SU(2)$ left-invariant one-forms in terms of the Euler angles, as in \eqref{eq:su2euler}. Upon doing so, the metric takes the following form
\begin{equation}\label{eq:gbexplicit}
g_{\mu\nu}=\left(
\begin{array}{cccc}
 1 & 0 & 0 & 0 \\
 0 & \frac{1}{4} \left(r^2+1\right) & 0 & 0 \\
 0 & 0 & \frac{1}{8} \left(-\cos (2 \theta )+2 r^2+1\right) & \frac{1}{4} r^2 \cos (\theta ) \\
 0 & 0 & \frac{1}{4} r^2 \cos (\theta ) & \frac{r^2}{4} \\
\end{array}
\right)
\end{equation}
This is not such a terribly complicated expression, and hence explicit computations can be carried out. As a side note, all of these computations can also be obtained by means of Cartan calculus, obtaining the curvature two-form, and so on. While this would involve less steps computationally, one must be more careful when setting up the flow equations. In any case, from \eqref{eq:gbexplicit} we can obtain the scalar curvature, as a kind of consistency check, since we know that this metric should describe a scalar-flat space. Indeed, we obtain 
\begin{equation}
    R=0
\end{equation}
identically.

In order to set up the usual Ricci flow equations, we need the Ricci tensor. For the Burns metric, in the above coordinates, it is
\begin{equation}\label{eq:Rbexplicit}
    R_{\mu\nu}=\left(
\begin{array}{cccc}
 -\frac{2}{\left(r^2+1\right)^2} & 0 & 0 & 0 \\
 0 & \frac{1}{2( r^2+1)} & 0 & 0 \\
 0 & 0 & \frac{2-2 \left(2 r^2+1\right) \cos (2 \theta )}{8 \left(r^2+1\right)^2} & -\frac{r^2 \cos (\theta )}{2 \left(r^2+1\right)^2} \\
 0 & 0 & -\frac{r^2 \cos (\theta )}{2 \left(r^2+1\right)^2} & -\frac{r^2}{2 \left(r^2+1\right)^2} \\
\end{array}
\right)
\end{equation}
Upon first inspection, this is a very nice result. If we compare \eqref{eq:Rbexplicit} with \eqref{eq:gbexplicit}, it appears as if $R_{\mu\nu}$ is proportional to $g_{\mu\nu}$, namely $R_{\mu\nu}=\Lambda g_{\mu\nu}$, which would mean that we are dealing with an Einstein manifold, and hence a Ricci soliton, whose behavior under the flow is easy to characterize. However, this is not the case. If we try to extract an overall constant from the Ricci tensor, we are left with 
\begin{equation}\label{eq:notasoliton}
    R_{\mu\nu}=\frac{2}{(1+r^2)^2}\left(
\begin{array}{cccc}
 -1 & 0 & 0 & 0 \\
 0 & \frac{1}{4} \left(r^2+1\right) & 0 & 0 \\
 0 & 0 & \frac{1}{8} \left(1-\left(2 r^2+1\right) \cos (2 \theta )\right) & -\frac{1}{4} r^2 \cos (\theta ) \\
 0 & 0 & -\frac{1}{4} r^2 \cos (\theta ) & -\frac{r^2}{4} \\
\end{array}
\right),
\end{equation}
and the leftover matrix is not directly proportional to the metric. 

Not deterred by this, we could relax our definition of a Ricci soliton or, rather, what we mean by saying that the Ricci tensor is proportional to the metric. We will try to give a general argument here. Let $g$ be some Riemannian metric, and $R$ its Ricci tensor, and suppose that the following relation holds
\begin{equation}\label{eq:lambdaNg}
    R=\Lambda Ng,
\end{equation}
where $N$ is some proportionality matrix. Then, the Ricci flow equations read
\begin{equation}\label{eq:notsoli}
    \frac{\partial g(t)}{\partial t}=-2\Lambda Ng(t).
\end{equation}
Because of the appearance of $g$ on the right hand side, these equations can be solved explicitly. With the initial condition $g(0)=g_0$, a solution for \eqref{eq:notsoli} is \footnote{This can be used to treat other metrics, such as the Eguchi-Hanson metric. Is this something worth including in an appendix?}
\begin{equation}
    g(t)=\exp\left(-2\Lambda Nt\right)g_0,
\end{equation}
where exp is understood as the matrix exponential. While this is not as simple as the equation for an Einstein manifold, it is still a closed equation (whenever the matrix exponential is), and in principle allows us to extract information about the evolution of the manifold in terms of the properties of $N$. If all else fails, one may always diagonalize $N$, and consider a new coordinate system, with simpler flow equations.

Let us now revisit the case for the Burns metric. Right off the bat, we can set\footnote{This looks very similar to the proportionality constant for the Witten cigar, is there a connection?} $\Lambda=2(1+r^2)^{-2}$, which is moreover strictly positive for all values of $r$. Then, from \eqref{eq:notasoliton}, and \eqref{eq:notsoli}, we can see that 
\begin{equation}
    N=\frac{1}{\Lambda}Rg^{-1}=\left(
\begin{array}{cccc}
 -1 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 \\
 0 & 0 & 1 & -2 \cos (\theta ) \\
 0 & 0 & 0 & -1 \\
\end{array}
\right)
\end{equation}
Not only is this matrix diagonalizable, it is idempotent. Indeed, $N^2=\mathbb{I}_4$. This straightforwardly implies that we have a closed expression for its exponential:
\begin{equation*}
    \exp(-2\Lambda Nt)=\begin{pmatrix}
    e^{2\Lambda t} & 0& 0& 0 \\
     0 & e^{-2\Lambda t} & 0 & 0 \\
 0 & 0 & e^{-2\Lambda t} & 2\sinh(2\Lambda t)\cos(\theta) \\
 0 & 0 & 0 & e^{2\Lambda t} \\
    \end{pmatrix}
\end{equation*}
Finally, the metric that solves the Ricci flow equations for the Burns metric is
\begin{equation*}
    g(t)=\left(
\begin{array}{cccc}
 e^{2 \Lambda  t} & 0 & 0 & 0 \\
 0 & \frac{1}{4} \left(r^2+1\right) e^{-2 \Lambda  t} & 0 & 0 \\
 0 & 0 & \frac{1}{4} \left(-\cos (2 \theta )+2 r^2 \cos ^2(\theta ) \sinh(2\Lambda t)+2 r^2+1\right) & \frac{1}{4} r^2 \cos (\theta ) e^{2 \Lambda  t} \\
 0 & 0 & \frac{1}{4} r^2 \cos (\theta ) e^{2 \Lambda  t} & \frac{1}{4} r^2 e^{2 \Lambda  t} \\
\end{array}
\right)
\end{equation*}
While more complicated than the original Burns metric, this is in the end a closed form of the metric along the flow. Therefore, we are able to carry out explicit computations. The expression for the Ricci tensor for the above metric is rather long and cumbersome, so we have decided not to include it here. For our end goal, it is enough to know the scalar curvature of the Burns metric along the flow. While at $t=0$ the geometry was scalar-flat, we now have that
\begin{equation}
    R(t)=-4\sinh(2\Lambda t) \frac{r^2 \left(e^{4 \Lambda  t}-3\right)-4}{\left(1+r^2\right)^2}.
\end{equation}
Note that $R(0)=0$ identically, as we expected.

The behavior that this result represents is interesting. Because $\lim_{t\to\infty}\sinh(2\Lambda t)=\infty$ when $\Lambda>0$, it is not hard to see that
\begin{equation}
    \lim_{t\to\infty}R(t)=-\infty, \hspace{0.5cm}\text{for all }r>0.
\end{equation}
On the other hand, at the origin (and only at the origin) we have that 
\begin{equation}
    \lim_{t\to\infty}R(t)|_{r=0}=\infty
\end{equation}
The origin (the location of the principal divisor) was precisely the point of interest for us, and we see that, at least for the Burns metric, the curvature blows up to infinity. By the discussion for the full $n\mathbb{CP}^2$ metric, we can justify that the whole manifold shrinks under the Ricci flow, leaving only the K3, with a set of points on it.

---------------------------------------------------

